Compressive Visual Representations

Learning effective visual representations that generalize well without human supervision is a fundamental problem in order to apply Machine Learning to a wide variety of tasks. Recently, two families of self-supervised methods, contrastive learning and latent bootstrapping, exemplified by SimCLR and BYOL respectively, have made significant progress. In this work, we hypothesize that adding explicit information compression to these algorithms yields better and more robust representations. We verify this by developing SimCLR and BYOL formulations compatible with the Conditional Entropy Bottleneck (CEB) objective, allowing us to both measure and control the amount of compression in the learned representation, and observe their impact on downstream tasks. Furthermore, we explore the relationship between Lipschitz continuity and compression, showing a tractable lower bound on the Lipschitz constant of the encoders we learn. As Lipschitz continuity is closely related to robustness, this provides a new explanation for why compressed models are more robust. Our experiments confirm that adding compression to SimCLR and BYOL significantly improves linear evaluation accuracies and model robustness across a wide range of domain shifts. In particular, the compressed version of BYOL achieves 76.0% Top-1 linear evaluation accuracy on ImageNet with ResNet-50, and 78.8% with ResNet-50 2x.

==> tables/imagenet_linear_eval_sota.tex <==
\begin{table}[tb]
  \caption{State-of-the-art comparison for linear evaluation of self-supervised representations on ImageNet. 
  Models are trained for 1000 epochs, except for those denoted by *, which were trained for 800 epochs by the original authors.
  \TODO{Two-column table? One for ResNet-50, and one for ResNet-50 2x}
  \KH{Can we actually drop ResNet-50 2x table? People look at R50 results for SoTA I think, and we have r50 2x in table 1. Then we can make this table parallel to table 2?}
  \ANURAG{Dropping R50-2x table is an option}
  \ANURAG{Where does 71.8 number for SwAV come from?}
  \ANURAG{We can maybe report SwAV 2-crop number only. And say in text that we don't report multi-crop, and that SwAV shows its complementary and brings improvements to multiple methods}
  }
  \centering
  \begin{tabular}{lcc}
  \toprule
  % \multicolumn{3}{l}{\textit{ResNet-50}} \\
  Method & Top 1 & Top 5 \\
  \midrule
  SimCLR \cite{chen2020simple}  & 69.3 & 89.0  \\
  MoCo v2* \cite{chen2020improved} & 71.1 & - \\
  InfoMin Aug* \cite{tian2020makes} & 73.0 & 90.1 \\
  SwAV* (2 crop) \cite{caron2020unsupervised,chen2020exploring}  & 71.8  & - \\
  Barlow Twins~\cite{zbontar2021barlow}  & 73.2 & 91.0 \\
  BYOL \cite{grill2020bootstrap}  & 74.3 & 91.6 \\
%   PIRL \cite{li2021prototypical} &  \\
  \midrule 
  C-SimCLR (ours)      & 71.5 & 90.6 \\
  C-BYOL (ours)        & \textbf{75.0} & \textbf{92.0} \\
  \midrule
  % SwAV* (multi-crop) \cite{caron2020unsupervised}  & 75.3  & - \\
  % \midrule
  Supervised baseline \cite{chen2020simple} & 76.0 & 93.1 \\
  \bottomrule
  \end{tabular}
    
  \label{tab:linear_eval_sota}
\end{table}

\iffalse
    \begin{table}
      \caption{Linear evaluation (1000 epochs). Show accuracy delta. Do 3 runs if we have time.}
      \centering
    %   \begin{tabular}{lllllllllll}
      \begin{tabular}{llllll}
        \toprule
         & & \multicolumn{2}{c}{Uncompressed} & \multicolumn{2}{c}{Compressed} \\
        Method  & Architecture  & Top-1 & Top-5 & Top-1 & Top-5 \\
        \midrule
        Supervised baseline \\
        SimCLR \cite{chen2020simple}  & ResNet-50 & 69.3 & 89.0 \\
        SimCLR \cite{chen2020simple}  & ResNet-50 2x & 74.2 & 92.0 \\
        BYOL \cite{grill2020bootstrap}  & ResNet-50 & 74.3 & 91.6 \\
        BYOL \cite{grill2020bootstrap}  & ResNet-50 2x & 77.4 & 93.6 \\
        SimCLR*  & ResNet-50 & 70.7 & 90.2 & 71.5 (+0.8) & 90.5 (+0.3)    \\
        SimCLR*   & ResNet-50 2x & 74.3 & 92.0 & 74.9 & 92.3 \\
        BYOL & ResNet-50    \\
        BYOL & ResNet-50 2x    \\
        MoCo v2-800epochs \cite{chen2020improved} & ResNet-50 & 71.1 & - \\
        CPC v2 \cite{henaff2020data} \\
        PIRL \cite{li2021prototypical} \\
        InfoMin Aug \\
        SwAV & ResNet-50 &  &  \\
        \midrule
        & ResNet-152?    \\
        \bottomrule
      \end{tabular}
        \label{tab:linear_eval_sota}
    \end{table}
\fi

==> text/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\iffalse
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\fi

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \Cref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \Cref{sec:conclusion}.}
    % Same as any other image representation learning paper ... Image representations could be misued ... Training datasets (like ImageNet) have biases that are not suitable for all applications. People could misuse models (intentionally or not) to make decisions that impact different groups in society differently
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerNA{No assumptions.}
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See \Cref{sec:complete_lipschitz}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    % \answerTODO{Code will be released upon acceptance.}
    \answerNo{As mentioned in Section~\ref{sec:experiments_setup}, we will release code and models upon acceptance. All data is already public.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \Cref{sec:experiments_setup} and \Cref{sec:impl_detail}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See \Cref{sec:experiments_setup}. As in \cite{grill2020bootstrap}, we report our accuracies averaged over three pretraining trials for the main results but omit error bars in reporting for readability because we found the maximum absolute difference between the best and worst trials to be less than 0.15 for 1000-epoch models and 0.27 for 300 epoch models.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{As described in \Cref{sec:experiments_setup}, we used Google Cloud TPU v3 accelerators, with 64 cores per experiment.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


